Unraveling the Never-Ending Story of Lifecycles and Vitalizing Processes

Business process management (BPM) has been widely used to discover, model, analyze, and optimize organizational processes. BPM looks at these processes with analysis techniques that assume a clearly defined start and end. However, not all processes adhere to this logic, with the consequence that their behavior cannot be appropriately captured by BPM analysis techniques. This paper addresses this research problem at a conceptual level. More specifically, we introduce the notion of vitalizing business processes that target the lifecycle process of one or more entities. We show the existence of lifecycle processes in many industries and that their appropriate conceptualizations pave the way for the definition of suitable modeling and analysis techniques. This paper provides a set of requirements for their analysis, and a conceptualization of lifecycle and vitalizing processes.

==> 5-exploratory-case-study.tex <==
\section{Validation}
\label{sec:casestudy}















In this section, we validate the formal modelling of lifecycle process. Thus, we  map the formal concepts on to the MIMIC-IV dataset~\cite{johnson_mimic-iv_2023} ending with discussing the implications from this mapping.x
The MIMIC-IV dataset was considered for traditional process mining in previous work by Cremerius et al.~\cite{DBLP:conf/icpm/CremeriusPKW22}.
To exemplify the application of our concept, let us consider the case of a chronic disease treatment, such as lower back pain. A patient affected by such a disease needs to undergo regular treatment in the hospital.
In the MIMIC-IV dataset we observe the related \textit{lifecycle history} of the entity \verb|patient| that is identifiable through a \verb|subject_id|, that will serve as our entity id $\epsilon$. Let us consider the patient with entity id $ \epsilon = 10013310$.
The table \verb|edstays| captures the different stays of a patient, each belonging to a different vitalizing case id $c$.

\textbf{Event sequence}. 
The universe of events $\mathcal{E}$ is mapped to all the entries that have a timestamp in any table of MIMIC-IV -- most of the MIMIC-IV tables contain events, such as the table \verb|procedureevents|, \verb|Ingredientevents|, and \verb|medrecon|.
$\mathcal{A}$ -- the universe of actions -- is mapped to all the medicament related recordings. These can be found in the tables \verb|prescriptions|, \verb|pharmacy|,  \verb|emar|,  and \verb|emar_details|.
For what concerns $\mathcal{I}$, $\mathcal{T}$ and $\Xi$ -- respectively the event indicators, timestamps and entity identifiers -- they are mapped by the specific attributes reported in the MIMIC-IV tables. 
$\mathcal{C}$ -- the universe of vitalizing case identifiers -- is related to the specific stays of a patient. In theory, vitalizing cases could also be defined my fine granular based on the different diagnosis. The diagnosis information could be retrieved from the \verb|diagnosis| table.
Then, an event $e \in \mathcal{E}$ is the instance $e =( i,a,t,\epsilon, c) =$ (\verb|event_id|, \verb|'pain'|, $2153-05-26 08:56:00$, $10013310$, \verb|vitalizing_case_id)| where \verb|event_id| is the unique identifier of the event id the database table

\textbf{Vital signs}. 
Observations of vital signs can be found in various tables of the MIMIC dataset.  
These include the tables \verb|vitalsign|, \verb|chartevents|, and \verb|labevents|. 
Then, each vital sign observation can be instantiated as the tuple $v= ( 2153-05-26 14:42:00, 99.0000)$. The sequence of vital sign observations $V_1$ is then the sequence of all the events that have the same values for vital sign \verb|Sinus Rhythm| and entity id $ \epsilon = 10013310$. 

\textbf{State sequence}. 
In MIMIC-IV there are various tables and codes to report states of patients. 
The diagnosis of a patient can be the foundation of a state and can be found in the table \verb|diagnosis|. Based on the diagnosis of a patient and the vital signs of a patient, states such as \verb|In Recovery| can be formed in collaboration with medical experts.

\textbf{Lifecycle history}. 
Given the above instances of event sequence, vital sign and state sequence, the lifecycle history $h$ can be created. 
Then,  $\eta: \Xi \mapsto \mathcal{E}^* \times \mathcal{S}^* \times 2^\mathcal{V}$ can be computed through \verb|join| operations on the entity attribute (i.e., \verb|subject_id| in MIMIC-IV tables) across all the representative tables. In the above examples the entity id $ \epsilon = 10013310$

\paragraph{Discussion}
We can observe that our concepts can be mapped onto MIMIC-IV dataset. We apply our approach with a layman's understanding of medicine. We were able to map the different components of our formal model to the MIMIC-IV dataset. This means, that our conceptualization of lifecycle processes can be found in real-world settings and describes a valid subclass of business processes.
Based on such a dataset we will be able to develop novel analysis techniques. This will allow us, to have new techniques that all the requirements we explored in \autoref{sec:requirements}.









